Free-ATM: Exploring Unsupervised Learning on Diffusion-Generated Images with Free Attention Masks

Despite the rapid advancement of unsupervised learning in visual representation, it requires training on large-scale datasets that demand costly data collection, and pose additional challenges due to concerns regarding data privacy. Recently, synthetic images generated by text-to-image diffusion models, have shown great potential for benefiting image recognition. Although promising, there has been inadequate exploration dedicated to unsupervised learning on diffusion-generated images. To address this, we start by uncovering that diffusion models' cross-attention layers inherently provide annotation-free attention masks aligned with corresponding text inputs on generated images. We then investigate the problems of three prevalent unsupervised learning techniques ( i.e., contrastive learning, masked modeling, and vision-language pretraining) and introduce customized solutions by fully exploiting the aforementioned free attention masks. Our approach is validated through extensive experiments that show consistent improvements in baseline models across various downstream tasks, including image classification, detection, segmentation, and image-text retrieval. By utilizing our method, it is possible to close the performance gap between unsupervised pretraining on synthetic data and real-world scenarios.

==> table/all_tables2.tex <==
\begin{table}
   \begin{minipage}{0.48\textwidth}
    \vspace{-0.75cm}
   \scalebox{0.93}{
   \centering
      \tablestyle{2.6pt}{1.38}
       
         }
         \vspace{-0.2cm}  
         \caption{ Results on CIFAR-100 with \textbf{downstream-aware supervised pre-training}. C100: CIFAR100.}
         \vspace{+0.1cm}  
         \label{tab: pre-train CIFAR-100}
      \end{minipage}
      \hfill
        \begin{minipage}{0.48\textwidth}
         \vspace{-0.75cm}
      \scalebox{0.93}{
      \centering
      \tablestyle{2.6pt}{1.38}
      \begin{tabular}{c|c|cccc}
           \bottomrule[1pt] 
           \multirow{2}{*}{\makecell[c]{Data}} &\multirow{2}{*}{\makecell[c]{pre-trained \\on IN-1k?}}& \multicolumn{4}{c}{Syn. images amount}\\
           & & 0 & 1.2M & 2.4M & 4.0M  \\
      \hline
      (None) & & 69.29 & - & - & - \\
      IN-1K Syn & &  - & 87.98 & \highlight{88.39} & - \\
      IN-2K Syn & &  - & - & \highlight{88.57} & \highlight{88.91} \\
      \hline
      (None) & \checkmark & - & 88.07 & - & -  \\
    %   IN-1K Real + IN-2K Syn & - & - & -  \\
           \toprule[1pt]
         %   \bottomrule[1pt]
         \end{tabular} 
         }
         \vspace{-0.2cm}  
         \caption{Results on CIFAR-100 with \textbf{downstream-agnostic supervised pre-training}. Backbone: DeiT-S. } 
         \label{tab: pre-train imgnet deit}
        %  \vspace{-0.1cm}  
      \end{minipage}
   \hfill
   \begin{minipage}{0.48\textwidth}
   \scalebox{0.93}{
   \centering
      \tablestyle{2.6pt}{1.2}
      \vspace{+0.3cm} 
       \begin{tabular}{c|c|cccc}
           \bottomrule[1pt] 
           \multirow{2}{*}{\makecell[c]{Data}} & \multirow{2}{*}{\makecell[c]{pre-trained \\on IN-1k?}}& \multicolumn{4}{c}{Syn. images amount}\\
           & & 0 & 1.2M & 2.4M & 4.0M  \\
           \hline
           (None) & & 66.08 & - & - & - \\
        %   IN-1K Real & 81.30 & - & - & 82.44 & - & -  \\
           IN-1K Syn &  & - & 79.00 & 80.00 & - \\
           IN-2K Syn &  & - & - & 80.54 & 80.72 \\
           \hline
           (None) & \checkmark & 81.30 & - & - & - \\
           \hline
           IN-1K Syn & \checkmark & -& - & \highlight{81.78} & - \\
           IN-2K Syn & \checkmark & -& - & \highlight{81.87} & \highlight{81.91} \\
           \toprule[1pt]
         %   \bottomrule[1pt]
         \end{tabular} 
         }
         \vspace{-0.2cm}  
         \caption{Results for object detection on PASCAL VOC with \textbf{downstream-agnostic supervised pre-training}, all results are reported in AP$_{50}$.}
         \vspace{-0.5cm}  
         \label{tab: pre-train imgnet super}
      \end{minipage}
      \hfill
      \begin{minipage}{0.48\textwidth}
      \scalebox{0.93}{
      \centering
      \tablestyle{2.6pt}{1.38}
      \begin{tabular}{c|c|cccc}
           \bottomrule[1pt] 
           \multirow{2}{*}{\makecell[c]{Data}} & \multirow{2}{*}{\makecell[c]{pre-trained \\on IN-1k?}}& \multicolumn{4}{c}{Syn. images amount}\\
           & & 0 & 1.2M & 2.4M & 4.0M  \\
      \hline
      (None) &  & 66.08 & - & - & - \\
      IN-1K Syn &  & - & 81.55 & 82.13 & - \\
      IN-2K Syn &  & - & - & 82.22 & 82.29 \\
      \hline
      (None) &\checkmark & 82.44 & - & - & -  \\
      \hline
      IN-1K Syn & \checkmark & - & - & \highlight{82.47} &-      \\
    %   IN-1K Real + IN-2K Syn & - & - & -  \\
           \toprule[1pt]
         %   \bottomrule[1pt]
         \end{tabular} 
         }
         \vspace{-0.2cm}  
         \caption{Results for object detection on PASCAL VOC with \textbf{downstream-agnostic self-supervised pre-training (Moco v2)}, all results are reported in AP$_{50}$.  }
         \label{tab: pre-train imgnet moco}
         \vspace{-0.5cm}  
      \end{minipage}
      \label{tab: pre-train agnostic, voc}
  \end{table}

==> table/mae.tex <==
\begin{table}[t]
\begin{tabular}{l|c|c}
\hline\hline
                  & ImageNet  & ADE20K \\
                  & $acc$ &$miou$  \\
                  \hline
supervised        & 81.0      & 47.4   \\
real              & 83.6      & 48.1   \\
\hline
synthetic         & 82.5      & 47.6   \\
synthetic w/ mask & 83.0      & 48.0   \\
mix               & 83.9      & 48.5  \\
\hline
\hline
\end{tabular}
\label{MAE}
\caption{TBD}
\end{table}

==> table/mae_ablate.tex <==
\begin{table}[h]
\centering
\begin{tabular}{cccc}
\hline
\hline
          
   
     
& random  & all hard mask & balance (ours)\\

  \hline 
 &82.4 &82.7 &83.2

\\

\hline\hline
\end{tabular}
\label{ab_mae}

\caption{Using different mask strategies of MAE \cite{mae}.}
\end{table}

==> table/moco.tex <==
\begin{table}[]
\begin{tabular}{l|c|c|c}
\hline
\hline
                  & PASVOC & COCO & Citysapce \\
                  
                  & $AP^{b}_{50}$  & $AP^{b}$ & $miou$     \\
                  \hline
random ini        & 59.0   & 31.4 & 65.2      \\
supervised        & 81.6   & 39.2 & 74.2      \\
real              & 82.4   & 39.8 & 75.0
\\
\hline
synthetic         & 81.6   & 37.9 & 74.1      \\
synthetic w/ mask & 82.1     & 38.3 & 74.8      \\
mix               & 82.7   & 40.1 & 75.3 \\
\hline\hline
\end{tabular}
\label{results_moco}
\caption{TBD}
\end{table}

==> table/simclr.tex <==
\begin{table}[t]
\begin{tabular}{l|cc|c}
\hline
\hline
                  & \multicolumn{2}{c|}{COCO} & Cityspace \\
                  &    $AP^b$          & $AP^m$     & $miou$     \\
                  \hline
random ini        & 31.4        & 28.5       & 65.2      \\
supervised        & 39.2        & 35.5       & 74.2      \\
real              & 37.7        & 34.2       & 74.8      \\
\hline
synthetic         & 36.4        & 33.1       & 73.7      \\
synthetic w/ mask & 37.6        & 34.2       & 74.5      \\
mix               & 38.7          & 34.8       & 75.0       \\
\hline
\hline        
\end{tabular}
\label{simclr}
\caption{TBD}
\end{table}

==> table/svsu.tex <==
\begin{table}[h]
\centering
\begin{tabular}{ccc}
\hline
\hline
          
   
     
 & supervised  & unsupervised (ours) \\

  \hline 
 $AP^{b}_{50}$ &79.8 &82.1

\\

\hline\hline
\end{tabular}
\label{hhd}

\caption{Supervised vs unsupervised pretraining (ours) on synthetic images. }
\end{table}
